Variational quantum solutions to the Shortest Vector Problem

A fundamental computational problem is to find a shortest non-zero vector in Euclidean lattices, a problem known as the Shortest Vector Problem (SVP). This problem is believed to be hard even on quantum computers and thus plays a pivotal role in post-quantum cryptography. In this work we explore how (efficiently) Noisy Intermediate Scale Quantum (NISQ) devices may be used to solve SVP. Specifically, we map the problem to that of finding the ground state of a suitable Hamiltonian. In particular, (i) we establish new bounds for lattice enumeration, this allows us to obtain new bounds (resp.~estimates) for the number of qubits required per dimension for any lattices (resp.~random q-ary lattices) to solve SVP; (ii) we exclude the zero vector from the optimization space by proposing (a) a different classical optimisation loop or alternatively (b) a new mapping to the Hamiltonian. These improvements allow us to solve SVP in dimension up to 28 in a quantum emulation, significantly more than what was previously achieved, even for special cases. Finally, we extrapolate the size of NISQ devices that is required to be able to solve instances of lattices that are hard even for the best classical algorithms and find that with approximately $10^3$ noisy qubits such instances can be tackled.

==> experimental_results/convergence_times_plot.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[xlabel=Lattice rank, ylabel=Number of iterations]
		\addplot[blue, solid, mark=o]
		plot [error bars/.cd, y dir = both, y explicit]
		table[x =x, y =y, y error =e]{experimental_results/quantum_exp_data/convergence_times.txt};
		\end{axis}
	\end{tikzpicture}
	\caption{Averaged number of VQE iterations until convergence in our experiments with standard deviations\label{fig:convergence_rates}}
\end{figure} 

==> experimental_results/cvar_hit_rates.tex <==
\begin{figure}\label{fig:cvar_hit_rates}
	\centering
	\begin{tikzpicture}
				\begin{groupplot}[
			group style={
				group name=my plots,
				group size=1 by 3,
				ylabels at=edge left,
				vertical sep=1.5cm
			},
			footnotesize,
			width=15.5cm,
			height=7cm,
			tickpos=left,
			ytick align=outside,
			xtick align=outside,
			yticklabel style={
				/pgf/number format/fixed,
				/pgf/number format/precision=4,
			},
			scaled y ticks=false,
			enlarge x limits=false,
			ymin=0, ymax=0.61
			]
			\definecolor{mygr}{HTML}{2DA10B}
			
			\nextgroupplot[title={a)}, xlabel=Parameter $\alpha$, ylabel=Overlap with shortest lattice vector]

			\addplot[blue, solid, mark=o]
			plot [error bars/.cd, y dir = both, y explicit]
			table[x =x, y =y, y error =e]{experimental_results/quantum_exp_data/cvar_hit_rates.txt};
			
			\nextgroupplot[title={b)}, xlabel=Parameter $\alpha$, ylabel=Overlap with shortest lattice vector, ymin=0,ymax=0.007]
			\addplot[blue, solid, mark=o] table{experimental_results/quantum_exp_data/cvar_medians.txt};
			
			\nextgroupplot[title={c)}, xlabel=Parameter $\alpha$, ylabel=Probability of finding the ground state,ymin=0,ymax=1]
			\addplot[blue, solid, mark=o] table{experimental_results/quantum_exp_data/cvar_5000samples.txt};

		\end{groupplot}
	\end{tikzpicture}
	\caption{a) Averaged overlap of final ansatz with Hamiltonian's excited state corresponding to the shortest lattice vector with standard deviations as a function of parameter $\alpha$. b) Mean overlap of final ansatz with first excited state. c) Probability of obtaining a ground state with 5000 samples. Experiment was run for 1024 instances of lattices with rank 15.}
\end{figure} 

==> experimental_results/experimental_results.tex <==
\include{experimental_results/convergence_times_plot.tex}
\include{experimental_results/hit_rates.tex}

==> experimental_results/hit_rates.tex <==
\begin{figure}[H]
	\centering
	\begin{tikzpicture}
		\begin{axis}[xlabel=Lattice rank, ylabel=Overlap with the shortest lattice vector,	yticklabel style={
				/pgf/number format/fixed,
				/pgf/number format/precision=4,
			},
			scaled y ticks=false]
		\addplot[blue, solid, mark=o]
		plot [error bars/.cd, y dir = both, y explicit]
		table[x =x, y =y, y error =e]{experimental_results/quantum_exp_data/hit_rates.txt};
		\end{axis}
	\end{tikzpicture}
	\caption{Averaged overlap of final ansatz with Hamiltonian's excited state corresponding to the shortest lattice vector with standard deviations\label{fig:hit_rates}}
\end{figure} 
